Prior preferences in active inference agents: soft, hard, and goal shaping

Active inference proposes expected free energy as an objective for planning and decision-making to adequately balance exploitative and explorative drives in learning agents. The exploitative drive, or what an agent wants to achieve, is formalised as the Kullback-Leibler divergence between a variational probability distribution, updated at each inference step, and a preference probability distribution that indicates what states or observations are more likely for the agent, hence determining the agent's goal in a certain environment. In the literature, the questions of how the preference distribution should be specified and of how a certain specification impacts inference and learning in an active inference agent have been given hardly any attention. In this work, we consider four possible ways of defining the preference distribution, either providing the agents with hard or soft goals and either involving or not goal shaping (i.e., intermediate goals). We compare the performances of four agents, each given one of the possible preference distributions, in a grid world navigation task. Our results show that goal shaping enables the best performance overall (i.e., it promotes exploitation) while sacrificing learning about the environment's transition dynamics (i.e., it hampers exploration).

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%
% Adjusted and extended from https://github.com/goodfeli/dlbook_notation.

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
%\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
	#1\;\delimsize\|\;#2%
}
\newcommand{\infdiv}{\KL \infdivx}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%%%% Commands below added by Filippo Torresan and Manuel Baltieri %%%%
% In-text comments
\newcommand{\comm}[1]{\textcolor{OrangeRed}{[#1]}}
% Definitions, Propositions, Principles, and Theorems (all requiring amsthm)
% Definition
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\theoremstyle{plain}
\newtheorem{proposition}{Proposition}[section]
\theoremstyle{plain}
\newtheorem{principle}{Principle}[section]
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\theoremstyle{definition}
\newtheorem{remark}{Remark}[section]
\tcolorboxenvironment{remark}{colframe=ForestGreen,breakable,before skip=10pt,after skip=10pt}

\newtheorem{example}[theorem]{Example}



\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

% For argmax and argmin operators
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% For probabilistic independence and dependence symbols
\newcommand{\indep}{\perp\!\!\!\!\perp}
\newcommand{\nindep}{\centernot{\indep}}

% backward blocking
\newcommand{\CueOne}{\mathbf{C}_1}
\newcommand{\CueTwo}{\mathbf{C}_2}
\newcommand{\Outcome}{\mathbf{+}}

% maths
\newcommand{\N}{\mathbb{N}}
\newcommand{\id}{\mathsf{id}}
\newcommand{\card}[1]{\lvert{#1}\rvert}
\newcommand{\prob}[1]{P(#1)}
\newcommand{\condprob}[2]{P({#1}|{#2})}
\newcommand{\definedas}{\doteq}

% POMDP
\newcommand{\statespace}{\mathcal{S}}
\newcommand{\obsspace}{\mathcal{O}}
\newcommand{\actionspace}{\mathcal{A}}
\newcommand{\policyspace}{\Pi}
\newcommand{\Transition}{\mathcal{T}}
\newcommand{\Emission}{\mathcal{E}}
\newcommand{\ntime}{T}
\newcommand{\horizon}{H}
\newcommand{\action}{a}
\newcommand{\ohaction}{\mathbf{\mathsf{a}}}
\newcommand{\actionvar}{A}
\newcommand{\state}{s}
\newcommand{\ohstate}{\mathbf{\mathsf{s}}}
\newcommand{\statevar}{S}
\newcommand{\obs}{o}
\newcommand{\ohobs}{\mathbf{\mathsf{o}}}
\newcommand{\obsvar}{O}
\newcommand{\tprob}[1]{P({#1}| \state_{t}, \action_{t})}
\newcommand{\eprob}[1]{P({#1}| \state_{t})}

% Active inference
\newcommand{\fe}{\mathcal{F}}
\newcommand{\efe}{\mathcal{G}}
\newcommand{\totefe}{\mathcal{G}_{\polhorizon}}
\newcommand{\kldiv}{\mathcal{D}_{KL}}
\newcommand{\pprob}[1]{P^{*}({#1})}
\newcommand{\stateparams}{\mathbf{s}}
\newcommand{\obsparams}{\mathbf{o}}
\newcommand{\policyparams}{\boldsymbol{\policy}}
\newcommand{\seqstates}[1]{\state_{1}, \dots, \state_{{#1}}}
\newcommand{\seqobs}[1]{\obs_{1}, \dots, \obs_{{#1}}}
\newcommand{\seqactions}[1]{\action_{1}, \dots, \action_{{#1}}}
\newcommand{\decision}{d}
\newcommand{\genmodel}{\mathcal{M}}
\newcommand{\gmparams}{\boldsymbol{\Theta}}
\newcommand{\varapprox}{\mathcal{V}}
\newcommand{\seqv}[3]{{#1}_{#2:#3}}
\newcommand{\policy}{\pi}
\newcommand{\polhorizon}{H}
\newcommand{\numpolicies}{\mathtt{p}}
\newcommand{\obsmap}{\mathbf{A}}
\newcommand{\transmap}{\mathbf{B}}
\newcommand{\tprobaif}{P(\statevar_{t}| \statevar_{t-1}, \policy, \transmap)}
\newcommand{\eprobaif}{P(\obsvar_{t}| \statevar_{t-1}, \obsmap)}
\newcommand{\varprob}[1]{Q(#1)}
\newcommand{\softmax}[1]{\sigma(#1)}
\newcommand{\entropy}{\mathbb{H}}

% RL
\newcommand{\actions}{\mathbf{a}}
\newcommand{\Actions}{A}
\newcommand{\reward}{r}
\newcommand{\Reward}{R}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Observations}{M}
\newcommand{\stateaction}{\tau}
\newcommand{\obsaction}{\tau^{\text{POMDP}}}
\newcommand{\policyparameters}{{\boldsymbol{\theta}}}
\newcommand{\Advantage}{\text{Adv}}
\newcommand{\return}{G}
\newcommand{\expreturn}{J}
\newcommand{\valuefunction}{V}
\newcommand{\beliefs}{B}

% actor-critic
\newcommand{\behavioural}{{\boldsymbol{\beta}}}
\newcommand{\importanceweights}{{\boldsymbol{w}_{T}^{i}}}
\newcommand{\discount}{\gamma}
\newcommand{\estexpreturn}{\hat{\expreturn}}
\newcommand{\Qfunction}{Q}
\newcommand{\ntrajectories}{N}

\newcommand{\itertrajectories}{n}
\newcommand{\itertime}{t}
\newcommand{\iterpartial}{i}

% scm
\newcommand{\noise}{N}
\newcommand{\scm}{\mathcal{C}}
\newcommand{\assignment}{h}
\newcommand{\emission}{g}
\newcommand{\PA}{\mathbf{PA}}

\newcommand{\confounders}{\mathbf{c}}
\newcommand{\Confounders}{C}
\newcommand{\nconfounders}{m}


% autoencoder
\newcommand{\Data}{\mathcal{D}}
\newcommand{\encoderweights}{\boldsymbol{\phi}}
\newcommand{\decoderweights}{\boldsymbol{\theta}}
\newcommand{\ELBO}{\mathcal{L}}
\newcommand{\VAELoss}{\ELBO}


%*********************************************************************************
% Listings Settings
%*********************************************************************************

% Setting the format for all the codes in line and float objects with \lstset
\lstset{language=Python,
	keywordstyle=\color{Plum},%\bfseries,
	basicstyle=\normalsize \ttfamily,
	identifierstyle=\color{Black},
	commentstyle=\color{Gray}\ttfamily,
	stringstyle= \color{LimeGreen} \rmfamily,
	numbers=left,%left,%
	numberstyle=\scriptsize, %\tiny %
	stepnumber=1,
	numbersep=8pt,
	%showstringspaces=false,
	%breaklines=true,
	%frameround=ftff,
	frame=single,
	%backgroundcolor = \color{},
	keepspaces=true
}

% Custom environment for all the codes in display in Python
\lstnewenvironment{Python}{\lstset{language=Python,
		keywordstyle=\color{Plum},%\bfseries,
		basicstyle=\small \ttfamily,
		identifierstyle=\color{Black},
		commentstyle=\color{Gray}\ttfamily,
		stringstyle= \color{LimeGreen} \rmfamily,
		numbers=left,%left,%
		numberstyle=\scriptsize, %\tiny
		stepnumber=1,
		numbersep=8pt,
		%showstringspaces=false,
		%breaklines=true,
		%frameround=ftff,
		frame=none,
		%backgroundcolor = \color{},
		keepspaces=true
	}}{}

% new listing object with tcolorbox package
\newtcblisting[auto counter, number within=section]{code}[2][]{
	fonttitle=\bfseries, colback=black!5!white, colframe=black!73!white, listing only,
	listing options={
			language=Python,
			keywordstyle=\color{Plum},%\bfseries,
			basicstyle=\normalsize \ttfamily,
			identifierstyle=\color{Black},
			commentstyle=\color{Gray}\ttfamily,
			stringstyle= \color{LimeGreen} \rmfamily,
			numbers=left,%left,%
			numberstyle=\scriptsize, %\tiny
			stepnumber=1,
			numbersep=8pt,
			%showstringspaces=false,
			%breaklines=true,
			%frameround=ftff,
			frame=none,
			%backgroundcolor = \color{},
			keepspaces=true},
	title=Code \thetcbcounter: #2, #1}

% new tcolorbox object for pseudocode with algorithm2e
% Argument #2 corresponds to the title for the box, argument #1 is optional and will add a label if given
% Example: \begin{pscode}[label={pscode:aaa}]{Pscode One}

\newtcolorbox[use counter=pscode, list inside = boxes]{pscode}[2][]{
	fonttitle=\bfseries,
	colback=black!5!white,
	colframe=black!73!white,
	before upper={\begin{algorithm}[H]},
				after upper={\end{algorithm}},
	%floatplacement=tb, float,
	title=Algorithm \thepscode: #2, #1}

% Define the counter to avoid "! LaTeX Error: No counter 'pscode' defined." when the counter is not
% automatically created, e.g., because there are no pscode environments in the main texts, triggering
% the error when we use \setcounter{pscode}{0} (but no counter exists) as part of \beginsupplement (see araya.csl)
\newcounter{pscode}
\crefname{pscode}{Algorithm}{Algorithms}
\Crefname{pscode}{Algorithm}{Algorithms}


% Example LaTeX code (to be copied and modified for a specific case)
%\begin{pscode}[label={pscode:perc-inf}]{Perceptual Inference}
%  \DontPrintSemicolon
%  \KwData{sensory observations, i.e.\ $o_{1}, \dots, o_{t}$, and policies $\pi_{1} \dots \pi_{n}$.}
%  \KwResult{updated beliefs about the states, i.e.\ $Q(S_{1}|\pi), \dots, Q(S_{T}|\pi)$.}
%  \BlankLine
%  \For{$\pi_{i} \in [\pi_{1} \dots \pi_{n}]$}{
%    \While{$ \mathcal{F}_{\pi_{i}} > \epsilon$}{
%      \For{$t \in [1 \dots T]$}
%      {$\mathbf{s}^{\pi_{i}}_{t} := \mathbf{s}^{\pi_{i}}_{t} - \nabla_{\mathbf{s}^{\pi_{i}}_{t}} \mathcal{F}_{\pi_{i}}$}
%    }}
%\end{pscode}

% new theorem box with tcolorbox package
\newtcbtheorem[auto counter, number within=section, list inside = boxes]{mytheo}{My Theorem}%
{colback=green!5,colframe=green!35!black,fonttitle=\bfseries}{th}

